Towards Large Reasoning Models: A Survey of Reinforced Reasoning with Large Language Models

Language has long been conceived as an essential tool for human reasoning. The breakthrough of Large Language Models (LLMs) has sparked significant research interest in leveraging these models to tackle complex reasoning tasks. Researchers have moved beyond simple autoregressive token generation by introducing the concept of "thought" -- a sequence of tokens representing intermediate steps in the reasoning process. This innovative paradigm enables LLMs' to mimic complex human reasoning processes, such as tree search and reflective thinking. Recently, an emerging trend of learning to reason has applied reinforcement learning (RL) to train LLMs to master reasoning processes. This approach enables the automatic generation of high-quality reasoning trajectories through trial-and-error search algorithms, significantly expanding LLMs' reasoning capacity by providing substantially more training data. Furthermore, recent studies demonstrate that encouraging LLMs to "think" with more tokens during test-time inference can further significantly boost reasoning accuracy. Therefore, the train-time and test-time scaling combined to show a new research frontier -- a path toward Large Reasoning Model. The introduction of OpenAI's o1 series marks a significant milestone in this research direction. In this survey, we present a comprehensive review of recent progress in LLM reasoning. We begin by introducing the foundational background of LLMs and then explore the key technical components driving the development of large reasoning models, with a focus on automated data construction, learning-to-reason techniques, and test-time scaling. We also analyze popular open-source projects at building large reasoning models, and conclude with open challenges and future research directions.

==> table_post-training.tex <==
\begin{table}[h]
\centering
\caption{Train-time reinforcement for LLM reasoning.}
\label{tab:my-table}
\resizebox{\textwidth}{!}{
\begin{tabular}{@{}cccccc@{}}
\toprule
Approach                    & Label                    & Paper                    & Year                 & Task                                                                                                       & Technique                                                               \\ \midrule
\multirow{5}{*}{Human}      & \multirow{1}{*}{Outcome} & \cite{nasution2024chatgpt}                  &          2024   &    Annotation quality  & Comparative analysis                                                                         \\ \cmidrule(l){2-6} 
                               
                            & \multirow{3}{*}{Process} & \cite{lightman2023let}   & 2023                 &  Reasoning                                                                                       & Manual labeling                                                        \\ \cmidrule(l){3-6} 
                            &                          & \cite{wang2024human}                  &     2024      &  Annotation   &  Collaborative verification                                                                                   \\ \midrule
\multirow{10}{*}{Automated} & \multirow{5}{*}{Outcome} & \cite{puri2020training}  &  2020   &  Questioning and answering     
                                                                    &   Text extraction                   
                                \\ \cmidrule(l){3-6} 
                            &            & \cite{schick2024toolformer} &     2024   &   Tool use                                     &  Matching
                            
                            %     \\ \cmidrule(l){3-6} 
                            % &            & \cite{goel2023llms}     &   2023    &  Medical Text Annotation              &   Two-stage Collaboration  
                            
                                \\ \cmidrule(l){3-6} 
                                
                            &            & \cite{wang2024human}     &   2024    & Text classification            &   Two-stage Collaboration  
                                \\ \cmidrule(l){3-6} 
                                
                            &            & \cite{li2023coannotating}   &  2023  & \begin{tabular}[c]{@{}c@{}}Topic classification\\ Semantic similarity\\ Nuanced comprehension   \end{tabular}
                                         & \begin{tabular}[c]{@{}c@{}}Task allocation\\ Uncertainty assessment\end{tabular}
                            
                                \\ \cmidrule(l){3-6} 
                            &                          & \cite{lee2024llm2llm} &  2024                      &      \begin{tabular}[c]{@{}c@{}}Math problems\\ Law cited cases\\ Text classification   \end{tabular}                                                                 &   Error correction
                                \\ \cmidrule(l){3-6} 
                            &                          & \cite{song2024trial}    &   2024                   &    \begin{tabular}[c]{@{}c@{}}Web navigation\\  Embodied  tasks\end{tabular}   &    Contrastive learning  
                                \\ \cmidrule(l){3-6} 
                            &                          & \cite{kwon2024language}    &   2024                   &   Everyday manipulation tasks   &    Synthetic augmentation
                                \\ \cmidrule(l){3-6} 
                            &                          & \cite{qiao2024autoact}    &   2024                   &    \begin{tabular}[c]{@{}c@{}}HotpotQA\\ScienceQA \end{tabular}  &    Multi-agent collaboration

                            
                            
                                                                        \\ \cmidrule(l){2-6} 
                            & \multirow{5}{*}{Process} & \cite{luo2023wizardmath} & 2023                 & Math problems                                                                                              & External LLM                                                             \\ \cmidrule(l){3-6} 
                            &                          & \cite{wang2024math}      & 2024                 & Math problems                                                                                              & Random simulation                                                       \\ \cmidrule(l){3-6} 
                            &                          & \cite{wang2024multi}     & 2024                 & \begin{tabular}[c]{@{}c@{}}Math problems\\ Programming\end{tabular}                                        & Random simulation                                                       \\ \cmidrule(l){3-6} 
                            &                          & \cite{luo2024improve}    & 2024                 & Math problems                                                                                              & MCTS simulation                                                         \\ \cmidrule(l){3-6} 
                            &                          & \cite{zhang2024rest}     & 2024                 & \begin{tabular}[c]{@{}c@{}}Math problems\\ Questioning and answering\\ Multi-domain knowledge reasoning\end{tabular} & \begin{tabular}[c]{@{}c@{}}MCTS simulation\\ Self-refining\end{tabular} \\ \bottomrule
\end{tabular}}
\end{table}
